HH-PIM: Dynamic Optimization of Power and Performance with Heterogeneous-Hybrid PIM for Edge AI Devices

Processing-in-Memory (PIM) architectures offer promising solutions for efficiently handling AI applications in energy-constrained edge environments. While traditional PIM designs enhance performance and energy efficiency by reducing data movement between memory and processing units, they are limited in edge devices due to continuous power demands and the storage requirements of large neural network weights in SRAM and DRAM. Hybrid PIM architectures, incorporating non-volatile memories like MRAM and ReRAM, mitigate these limitations but struggle with a mismatch between fixed computing resources and dynamically changing inference workloads. To address these challenges, this study introduces a Heterogeneous-Hybrid PIM (HH-PIM) architecture, comprising high-performance MRAM-SRAM PIM modules and low-power MRAM-SRAM PIM modules. We further propose a data placement optimization algorithm that dynamically allocates data based on computational demand, maximizing energy efficiency. FPGA prototyping and power simulations with processors featuring HH-PIM and other PIM types demonstrate that the proposed HH-PIM achieves up to $60.43$ percent average energy savings over conventional PIMs while meeting application latency requirements. These results confirm the suitability of HH-PIM for adaptive, energy-efficient AI processing in edge devices.

==> reference_name.tex <==
\if\useshortref 1

\newcommand{\DATE}{Proc. of DATE}
\newcommand{\ASPDAC}{Proc. of ASPDAC}
\newcommand{\DAC}{Proc. of DAC}
\newcommand{\ICCAD}{Proc. of ICCAD}
\newcommand{\ISCA}{Proc. of ISCA}
\newcommand{\NOCS}{Proc. of NOCS}
\newcommand{\HPCA}{Proc. of HPCA}
\newcommand{\IPDPS}{Proc. of IPDPS}
\newcommand{\ICCD}{Proc. of ICCD}
\newcommand{\MICRO}{Proc. of MICRO}
\newcommand{\ISQED}{Proc. of ISQED}
\newcommand{\CODES}{Proc. of CODES}
\newcommand{\RECONFIG}{Proc. ReConFig}
\newcommand{\SAMOS}{Proc. of SAMOS}
\newcommand{\ISLPED}{Proc. of ISLPED}
\newcommand{\ISVLSI}{Proc. of ISVLSI}
\newcommand{\ISSCC}{Proc. of ISSCC}
\newcommand{\PACT}{Proc. of PACT}
\newcommand{\COOLCHIPS}{Proc. of COOL Chips}
\newcommand{\ICECS}{Proc. of ICECS}
\newcommand{\HCS}{Proc. of HCS}
\newcommand{\SSS}{Proc. of S3S}
\newcommand{\ASAP}{Proc. of ASAP}
\newcommand{\SOFTCOM}{Proc. of SoftCOM}
\newcommand{\ICS}{Proc. of ICS}
\newcommand{\NOCARC}{Proc. of NoCArc}
\newcommand{\VLSID}{Proc. of VLSID}
\newcommand{\VLSISOC}{Proc. of VLSI-SoC}
\newcommand{\SOCC}{Proc. on SOCC}

\else

\if\usemiddleref 1

\newcommand{\DATE}{Proc. of Int. Conf. on Design, Automation \& Test in Europe}
\newcommand{\ASPDAC}{Proc. of Asia and South Pacific Design Automation Conference}
\newcommand{\DAC}{Proc. of Design Automation Conference}
\newcommand{\ICCAD}{Proc. of Int. Conf. on Computer-Aided Design}
\newcommand{\ISCA}{Proc. of Int. Symp. on Computer Architecture}
\newcommand{\NOCS}{Proc. of Int. Symp. on Networks-on-Chip}
\newcommand{\HPCA}{Proc. of Int. Symp. on High Performance Computer Architecture}
\newcommand{\IPDPS}{Proc. of Int. Parallel and Distributed Processing Symposium}
\newcommand{\ICCD}{Proc. of Int. Conf. on Computer Design}
\newcommand{\MICRO}{Proc. of Int. Symp. on Microarchitecture}
\newcommand{\ISQED}{Proc. of Int. Symp. on Quality Electronic Design}
\newcommand{\CODES}{Proc. of Int. Conf. on Hardware/Software Codesign and System Synthesis}
\newcommand{\RECONFIG}{Proc. of Int. Conf. on Reconfigurable Computing and FPGAs}
\newcommand{\SAMOS}{Proc. of Int. Conf. on Embedded Computer Systems}
\newcommand{\ISLPED}{Proc. of Int. Symp. on Low Power Electronics and Design}
\newcommand{\ISVLSI}{Proc. of IEEE Computer Society Annual Symposium on VLSI}
\newcommand{\ISSCC}{Proc. of Int. Solid-State Circuits Conference Digest of Technical Papers}
\newcommand{\PACT}{Proc. of Int. Conf. on Parallel Architecture and Compilation Techniques}
\newcommand{\COOLCHIPS}{Proc. of Symp. on Low-Power and High-Speed Chips and Systems}
\newcommand{\ICECS}{Proc. of Int. Conf. on Electronics, Circuits, and Systems}
\newcommand{\HCS}{Proc. of Hot Chips Symp.}
\newcommand{\SSS}{Proc. of S3S Conference}
\newcommand{\ASAP}{Proc. of Int. Conf. on Application-specific Systems, Architectures and Processors}
\newcommand{\SOFTCOM}{Proc. of Int. Conf. on Software, Telecommunications and Computer Networks}
\newcommand{\ICS}{Proc. of Int. Conf. on Supercomputing}
\newcommand{\NOCARC}{Proc. of Int. Workshop on Network on Chip Architectures}
\newcommand{\VLSID}{Proc. of Int. Conf. on VLSI Design}
\newcommand{\VLSISOC}{Proc. of Int. Conf. on VLSI and SoC}
\newcommand{\SOCC}{Proc. on Int. Symp. on SoC}

\else

\newcommand{\DATE}{Proceedings of the International Conference on Design, Automation \& Test in Europe}
\newcommand{\ASPDAC}{Proceedings of the Asia and South Pacific Design Automation Conference}
\newcommand{\DAC}{Proceedings of the Design Automation Conference}
\newcommand{\ICCAD}{Proceedings of the International Conference on Computer-Aided Design}
\newcommand{\ISCA}{Proceedings of the International Symposium on Computer Architecture}
\newcommand{\NOCS}{Proceedings of the International Symposium on Networks-on-Chip}
\newcommand{\HPCA}{Proceedings of the International Symposium on High Performance Computer Architecture}
\newcommand{\IPDPS}{Proceedings of the International Parallel and Distributed Processing Symposium}
\newcommand{\ICCD}{Proceedings of the International Conference on Computer Design}
\newcommand{\MICRO}{Proceedings of the International Symposium on Microarchitecture}
\newcommand{\ISQED}{Proceedings of the International Symposium on Quality Electronic Design}
\newcommand{\CODES}{Proceedings of the International Conference on Hardware/Software Codesign and System Synthesis}
\newcommand{\RECONFIG}{Proceedings of the International Conference on Reconfigurable Computing and FPGAs}
\newcommand{\SAMOS}{Proceedings of the International Conference on Embedded Computer Systems}
\newcommand{\ISLPED}{Proceedings of the International Symposium on Low Power Electronics and Design}
\newcommand{\ISVLSI}{Proceedings of the IEEE Computer Society Annual Symposium on VLSI}
\newcommand{\ISSCC}{Proceedings of the International Solid-State Circuits Conference Digest of Technical Papers}
\newcommand{\PACT}{Proceedings of the International Conference on Parallel Architecture and Compilation Techniques}
\newcommand{\COOLCHIPS}{Proceedings of the Symposium on Low-Power and High-Speed Chips and Systems}
\newcommand{\ICECS}{Proceedings of the International Conference on Electronics, Circuits, and Systems}
\newcommand{\HCS}{Proceedings of IEEE Hot Chips Symposium}
\newcommand{\SSS}{Proceedings of IEEE SOI-3D-Subthreshold Microelectronics Technology Unified Conference}
\newcommand{\ASAP}{Proceedings of International Conference on Application-specific Systems, Architectures and Processors}
\newcommand{\SOFTCOM}{Proceedings of International Conference on Software, Telecommunications and Computer Networks}
\newcommand{\ICS}{Proceedings of the International Conference on Supercomputing}
\newcommand{\NOCARC}{Proceedings of the International Workshop on Network on Chip Architectures}
\newcommand{\VLSID}{Proceedings of the International Conference on VLSI Design}
\newcommand{\VLSISOC}{Proceedings of International Conference on VLSI and System-on-Chip}
\newcommand{\SOCC}{Proceedings on International Symposium on System-on-Chip}

\fi
\fi

\if\useshortref 1

\newcommand{\TCAD}{IEEE TCAD}
\newcommand{\TVLSI}{IEEE TVLSI}
\newcommand{\TC}{IEEE TC}
\newcommand{\TPDS}{IEEE TPDS}
\newcommand{\TODAES}{ACM TODAES}
\newcommand{\TECS}{ACM TECS}
\newcommand{\JSSC}{IEEE JSSC}
\newcommand{\JMICRO}{IEEE MICRO}
\newcommand{\TCASI}{IEEE TCS-I}
\newcommand{\IEEE}{Proc. IEEE}
\newcommand{\SSCM}{IEEE SSC-M}
\newcommand{\IOTJ}{IEEE IoT}
\newcommand{\TMC}{IEEE TMC}
\newcommand{\IETCPS}{IET CPS}
\newcommand{\INTEGRATION}{Integration}
\newcommand{\ACCESS}{IEEE Access}

\else

\if\usemiddleref 1

\newcommand{\TCAD}{IEEE Trans. on Computer-Aided Design of Integrated Circuits and Systems}
\newcommand{\TVLSI}{IEEE Trans. on Very Large Scale Integration Systems}
\newcommand{\TC}{IEEE Trans. on Computers}
\newcommand{\TPDS}{IEEE Trans. on Parallel and Distributed Systems}
\newcommand{\TODAES}{ACM Trans. on Design Automation of Electronic Systems}
\newcommand{\TECS}{ACM Trans. on Embedded Computing Systems}
\newcommand{\JSSC}{IEEE Journal of Solid-State Circuits}
\newcommand{\JMICRO}{IEEE Micro}
\newcommand{\TCASI}{IEEE Trans. on Circuits and Systems I: Regular Papers}
\newcommand{\IEEE}{Proceedings of the IEEE}
\newcommand{\SSCM}{IEEE Solid-State Circuits Magazine}
\newcommand{\IOTJ}{IEEE Internet of Things Journal}
\newcommand{\TMC}{IEEE Trans. on Mobile Computing}
\newcommand{\IETCPS}{IET Cyber-Physical Systems}
\newcommand{\INTEGRATION}{Integration}
\newcommand{\ACCESS}{IEEE Access}

\else

\newcommand{\TCAD}{IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}
\newcommand{\TVLSI}{IEEE Transactions on Very Large Scale Integration Systems}
\newcommand{\TC}{IEEE Transactions on Computers}
\newcommand{\TPDS}{IEEE Transactions on Parallel and Distributed Systems}
\newcommand{\TODAES}{ACM Transactions on Design Automation of Electronic Systems}
\newcommand{\TECS}{ACM Transactions on Embedded Computing Systems}
\newcommand{\JSSC}{IEEE Journal of Solid-State Circuits}
\newcommand{\JMICRO}{IEEE Micro Magazine}
\newcommand{\TCASI}{IEEE Transactions on Circuits and Systems I: Regular Papers}
\newcommand{\IEEE}{Proceedings of the IEEE}
\newcommand{\SSCM}{IEEE Solid-State Circuits Magazine}
\newcommand{\IOTJ}{IEEE Internet of Things Journal}
\newcommand{\TMC}{IEEE Transactions on Mobile Computing}
\newcommand{\IETCPS}{IET Cyber-Physical Systems: Theory & Applications}
\newcommand{\INTEGRATION}{Integration the VSLI Journal}
\newcommand{\ACCESS}{IEEE Access}

\fi
\fi


==> tables/energy1.tex <==
%\begin{tabularx}{\textwidth}{C|C|C|C|C|C|C}
%\multicolumn{1}{c|}{}&\multicolumn{3}{c|}{50 MHz} & \multicolumn{3}{c}{100 MHz} \\
%\toprule
%%emp (${\degree}C$)&\textbf{Settling time ($s$)} & \textbf{Power ($mW$)} & \textbf{Energy ($Wh$)} & \textbf{Settling time (s)} & \textbf{Power ($mW$)}  & \textbf{Energy ($Wh$)} \\
%\toprule
%74	&577.29 & 1.47 & 777 & 577.29 & 3.58 & 777 \\
%\midrule
%79	&180.69 & 1.48 & 777 & 180.69 & 3.52 & 777 \\
%\bottomrule
%\end{tabularx}

{\color{black}
\begin{tabularx}{\textwidth}{C|C|C}
\toprule
&Clock frequency: 50MHz &Clock frequency: 100MHz\\
\midrule
$E_{Conv.}$ ($J$)&1.430&3.151\\
$E_{Proposed}$ ($J$)  &1.134 &2.455 \\
\midrule
Energy Saving (\%) &20.70 &22.09 \\
\bottomrule
\end{tabularx}
}

==> tables/exp_result.tex <==
\arrayrulecolor{black}
\begin{tabularx}{\textwidth}{c|C|C|C|C|C|C}
\toprule
Total Energy Consumption ($mJ$) & Case 1 & Case 2 & Case 3 & Case 4 & Case 5 & Case 6 \\
\midrule
Baseline PIM & 4.53 & 26.22 & 8.53 & 7.5 & 6.39 & 14.9 \\
\midrule
Hetero-PIM (w/o Data Placement) & 4.01 & 21.25 & 7.19 & 6.37 &  5.49 & 12.41 \\
\midrule
Hetero-PIM (with Data Placement) & 3.19 & 21.25 & 6.73 & 5.71 & 4.5 & 12.3 \\  
\bottomrule
\end{tabularx}

==> tables/param1.tex <==

\begin{tabularx}{\textwidth}{C|C|c|C|c|c|C}
\toprule
\multirow{2}{*}{\vspace{-1.2em}Power ($mW$)} & \multicolumn{2}{c|}{MRAM (128kB)} & \multicolumn{2}{c|}{SRAM (2kB)} & \multicolumn{2}{c}{PE}\\
\cmidrule{2-7}
 & Dynamic (Read/Write) & Static & Dynamic (Read/Write) & Static & Dynamic & Static \\
\midrule
HP-PIM ($V_{dd}=1.2V$) & 36.45 / 65.8 & 3.68 & 34.7 / 41.3 & 3.94 & 0.9 & 0.48\\
\midrule
LP-PIM ($V_{dd}=0.8V$) & 17.01 / 45.36  & 0.016 & 9.21 / 10.45 & 0.051 & 0.51 & 0.25\\            
\bottomrule
\end{tabularx}

%\begin{tabularx}{\textwidth}{C|C|C|C|C}
%\toprule
%\multirow{2}{*}{\vspace{-1.2em}Power ($mW$)} & \multicolumn{2}{c|}{MRAM (128kB)} & \multicolumn{2}{c}{SRAM (2kB)} \\
%\cmidrule{2-5}
% & Dynamic (Read/Write) & Static & Dynamic (Read/Write) & Static \\
%\midrule
%HP ($V_{dd}=1.2V$) & 145.81 / 263.21 & 14.736 & 145.81 / 263.21 & 14.736 \\
%\midrule
%LP ($V_{dd}=0.8V$) & 68.02 / 181.42  & 0.063 & 145.81 / 263.21 & 14.736 \\         
%\bottomrule
%\end{tabularx}


==> tables/param2.tex <==

\begin{tabularx}{\textwidth}{C|C|C|C|C|C}
\toprule
\multirow{2}{*}{\vspace{-1em}Latency ($ns$)} & \multicolumn{2}{c|}{MRAM} & \multicolumn{2}{c|}{SRAM} & \multirow{2}{*}{\vspace{-1em}PE}\\
\cmidrule{2-5}
 & Read & Write & Read & Write &  \\
\midrule
HP-PIM ($V_{dd}=1.2V$) & 2.27 & 6.17 & 0.46 & 0.46 & 4.72\\
\midrule
LP-PIM ($V_{dd}=0.8V$) & 3.44  & 7.16 & 0.89 & 0.89 & 7.42\\         
\bottomrule
\end{tabularx}

==> tables/resource.tex <==

\begin{tabular}{ll|c|c}

\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{IPs}} & {\multirow{2}{*}{ LUTs  }} & {\multirow{2}{*}{FFs}} \\
~ & ~ & ~  & ~ \\ \midrule  %\hline
\multicolumn{2}{c|}{RISC-V Rocket} & 11375 & 5762 \\ \midrule
\multicolumn{2}{c|}{Peripherals} & 5318 & 8607 \\ \midrule
\multicolumn{2}{c|}{System Interconnect} & 4624 & 6070 \\ \midrule
\multicolumn{2}{c|}{Heterogeneous PIM (PIM Module $\times 8$)} & 34757 & 13832 \\ %\cline{1-2}
~ &\multicolumn{1}{l|}{ $\bullet$ PIM Module}& 3809 & 1462 \\ 
~ & \multicolumn{1}{l|}{$\bullet$ PIM Controller} & 1767 & 871 \\\toprule

\end{tabular}


==> tables/time.tex <==

\arrayrulecolor{red}
\begin{tabularx}{\textwidth}{c|C|C|C|C|C}
\toprule
Execution Time ($\mu$$s$) & Level 1 & Level 2 & Level 3 & Level 4 & Level 5 \\
\midrule
$t_{constraint}$ & 300.00  & 128.57 & 90.00 & 64.29 & - \\
\midrule
HP-PIM & 0 & 12.43 & 27.91 & 38.05 & 45.41\\
\midrule
LP-PIM & 159.88  & 128.54 & 89.53 & 63.95 & 45.41\\
\bottomrule
\end{tabularx}

\arrayrulecolor{black}

